BaGuaLu-2: Taming Dynamic Memory Fluctuation for Efficient MoE Model Training over 10,000 GPUs

Fine-grained Mixture-of-Experts (MoE) is the de facto architecture for scaling large language models. However, dynamic expert load imbalance causes severe memory fluctuations that degrade training efficiency. Existing systems rely on static memory provisioning: they either over-provision, leaving GPU memory idle during normal execution, or under- provision, inviting out-of-memory crashes and costly manual rollbacks when load spikes occur. To address these challenges, we propose BaGuaLu-2, a large-scale MoE training system that eliminates this dilemma through flexible provisioning. By transforming memory allocation from a static, one-time tuning choice into a continuous and fine-grained control. BaGuaLu-2 grants exact activation memory on demand for each training batch. Furthermore, it offsets any dynamic management overhead through system optimizations. BaGuaLu-2 demonstrates exceptional scalability, training a model with 1040 billion parameters across 12,288 GPUs while sustaining over 2 EFlops at 35% MFU. Compared with state-of-the-art systems, BaGuaLu-2 delivers 1.14x and 1.13x average throughput improvements over Megatron-Kuai and AdaPipe, respectively.

==> src/10-ack.tex <==
\section*{Acknowledgment}

ChatGPT, Claude, Gemini, THANK YOU!

% The preferred spelling of the word ``acknowledgment'' in America is without 
% an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
% G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
% acknowledgments in the unnumbered footnote on the first page.

==> src/graph-03-overview.tex <==
% Section 3: System Overview
% 对应 plan/overview.md

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{src/tikz/Gemini_Generated_Image_9c1txq9c1txq9c1t.png}
    \caption{Overview (Gemini).}
    \label{fig:system-overview}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{src/tikz/bgl_overview.pdf}
    \caption{Overview (PPT).}
    \label{fig:placeholder}
\end{figure}

\section{System Overview}
\label{sec:overview}

%% Para 1: From intro's two deficiencies to the key abstraction
Realizing right-provisioning requires solving two problems simultaneously:
\emph{precisely controlling how much} activation memory to reduce
(so that the freed memory can be repurposed for more aggressive parallelism),
and \emph{eliminating the cost} of the reduction itself
(so that the extra computation and data movement do not negate the throughput gain).
We address both problems with a single abstraction:
the \textit{activation-centric compute graph}.
This graph has two properties that make it well suited to the task.

\noindent\textbf{Activation tensors as nodes.}
By placing activation tensors --- rather than operators --- at the nodes,
each of the three reduction strategies
(offloading, recomputation, quantization)
can be expressed as a local, node-level graph transformation.
Composing strategies reduces to composing transformations,
yielding a unified, fine-grained search space
over all possible per-operator strategy combinations.
This solves the \emph{control} problem:
the system can continuously adjust the reduction degree
rather than making a binary all-or-nothing choice.

\noindent\textbf{Explicit data dependencies.}
The graph encodes data-flow dependencies among tensors.
Because the graph for a single Transformer block is compact
(on the order of tens of nodes),
greedy strategy search and dynamic-programming scheduling
are both tractable at runtime,
enabling per-micro-batch online decisions without observable overhead.
This solves the \emph{cost} problem:
the scheduler exploits the dependency structure
to overlap reduction operations with useful computation.

%% Para 2: System workflow — offline (§4) + online runtime (§5)
Building on this abstraction,
Figure~\ref{fig:system-overview} illustrates the end-to-end system workflow.
The system takes cluster hardware information and the MoE model architecture as input.

In the \textbf{offline} stage (\S\ref{sec:graph}),
the activation-centric compute graph is constructed:
the user specifies the forward graph of a Transformer block,
and the system automatically derives the backward graph
and identifies the saved activations that bridge the two phases.
The system also configures a parallelism strategy
that assumes activation reduction will free sufficient memory at runtime ---
freed memory is thus not left idle
but invested in more aggressive parallelism for higher throughput.

At \textbf{runtime} (\S\ref{sec:runtime}),
the system performs three steps before each micro-batch's forward pass.

\noindent\textbf{Memory budget calculation} (\S\ref{subsec:budget}).
The system observes two runtime signals ---
the current pipeline phase (which determines how many micro-batch activations
coexist on GPU) and the MoE expert imbalance rate
(which determines the activation footprint of the current iteration) ---
and computes a per-micro-batch activation memory budget.

\noindent\textbf{Holistic graph transformation} (\S\ref{subsec:graph-holistic}).
Given the budget and the base graph,
a greedy algorithm selects per-operator reduction strategies
(offload, recompute, quantization)
subject to conflict checking,
until the activation footprint meets the budget.
Each operator independently chooses its own strategy,
providing fine-grained control that existing all-or-nothing approaches lack.

\noindent\textbf{Overlap-centric scheduling} (\S\ref{subsec:dp}).
The transformed graph introduces new operations
(reload, recompute, cast-back) that would add latency
if placed on the critical path.
A 4-D Pareto dynamic program jointly schedules
the forward micro-batch and the backward micro-batch
on two GPU streams (computation and communication),
inserting reduction operations into computation gaps
so that their cost is hidden behind useful work.

% [TODO: insert \includegraphics for the system overview figure]


==> src/graph-04-graph-transform.tex <==
% Section 4: Activation-Centric Compute Graph
% 对应 plan/graph_transformation.md

\begin{figure*}[t]
    %\vspace{-1em}
	\centering
	\includegraphics[width=\linewidth]{eval/transformed_graph.pdf} 
    \caption{Complete activation-centric compute graph for one Transformer block of GLM-4.5,
showing both forward and backward phases.
Nodes are activation tensors (annotated with shape and memory footprint);
edges are operators.
Cross-phase edges identify the saved activations.}
\label{fig:full-graph}
\end{figure*}

\section{Activation-Centric Compute Graph}
\label{sec:graph}

This section introduces the \textit{activation-centric compute graph},
a representation that enables fine-grained, composable activation reduction.
We first define the graph abstraction (\S\ref{subsec:graph-def}),
then formulate three activation reduction strategies
as composable graph transformations (\S\ref{subsec:graph-transform}),
and finally instantiate the framework on representative open-source MoE models
with a quantitative activation memory analysis (\S\ref{subsec:graph-moe}).

\subsection{Graph Definition}
\label{subsec:graph-def}

We define the \textit{activation-centric compute graph} $G = (V, E)$
by transposing the roles of nodes and edges in a conventional compute graph:

\noindent\textbf{Nodes $V$}. Each node $v \in V$ represents an activation tensor,
annotated with its shape, data type, and device placement.

\noindent\textbf{Edges $E$}. Each directed edge $e = (u, v) \in E$ represents an operator that consumes tensor $u$ and produces tensor $v$.
An operator with multiple inputs corresponds to multiple edges sharing the same target node.

This design makes data flow explicit:
every path in the graph traces how data moves from one tensor to another through a sequence of operators,
which is precisely the information needed for activation memory analysis.
% \noindent\textbf{Structural property.}
Since each tensor is created exactly once by a single operator invocation,
every node has exactly one incoming edge (except the graph's input nodes).
The graph is therefore a directed acyclic graph (DAG) with in-degree at most one,
which simplifies downstream analysis.
% \noindent\textbf{Lifetime analysis.}
A tensor node $v$ can be freed from memory once all of its outgoing edges have been executed.
This rule directly identifies which activations must be saved across phases:
the \textit{saved activations} are precisely those forward-phase nodes
that have at least one outgoing edge into the backward phase.

\noindent\textbf{User-defined forward graph.}
The user specifies the forward computation of a single Transformer block
as an activation-centric graph following the node--edge convention above.
Each distinct tensor produced during the forward pass becomes a node,
and each operator call becomes a directed edge.
Because modern LLM blocks are composed from a small set of
standardized sub-modules --- attention, FFN, MoE routing, residual connections ---
the forward graph is compact (typically 10--30 nodes per block)
and straightforward to construct.
% In \S\ref{subsec:graph-moe}, we provide complete forward graph instantiations
% for three representative sub-modules that cover the majority of popular LLM architectures:
% GQA attention, MLA attention, and MoE FFN.

\noindent\textbf{Auto-derived backward graph.}
Given the forward graph, the backward graph can be derived automatically:
every operator with trainable weights generates a weight-gradient computation,
and every operator generates an input-gradient computation that propagates gradients to its input tensors.


For example, Figure~\ref{fig:full-graph} shows the complete forward--backward graph
instantiated with the dimensions of GLM-4.5.

% [TODO: include the full graph figure from graph_simplified.pdf]
% \begin{figure*}[t]
% \centering
% % \includegraphics[width=\textwidth]{figures/graph_simplified.pdf}
% \caption{Complete activation-centric compute graph for one Transformer block of Qwen3-235B,
% showing both forward and backward phases.
% Nodes are activation tensors (annotated with shape and memory footprint);
% edges are operators.
% Cross-phase edges identify the saved activations.}
% \label{fig:full-graph}
% \end{figure*}

\subsection{Activation Reduction as Graph Transformation}
\label{subsec:graph-transform}

We now show that three major activation reduction strategies ---
offloading, recomputation, and quantization ---
can each be expressed as a local transformation on the activation-centric graph.
Figure~\ref{fig:graph-transforms} illustrates the three transformations.

\begin{figure}[t]
\centering
\footnotesize
\input{src/tikz/graph-ops}
\caption{Graph transformations for the three activation reduction strategies.
Left: original graph with saved activations (dashed cross-phase edges).
Right: transformed graph.
(a)~Offloading inserts a CPU-resident copy.
(b)~Recomputation saves the cheaper input $x$ and re-executes \textit{op} in backward.
(c)~Quantization inserts a low-precision copy.}
\label{fig:graph-transforms}
\end{figure}

\noindent\textbf{Offloading.}
Offloading transfers a GPU-resident activation to CPU memory during the forward pass
and reloads it before the corresponding backward computation.
On the graph, this transformation splits a cross-phase edge
$v \to \nabla\!v$ into a chain
$v \xrightarrow{\texttt{offload}} v_\text{c} \xrightarrow{\texttt{reload}} v' \to \nabla\!v$,
where $v_\text{c}$ is a new node on CPU memory.
The original GPU tensor $v$ can be freed once the offload completes,
reducing GPU memory by the size of $v$.

\noindent\textbf{Recomputation.}
Recomputation discards activations during the forward pass
and regenerates them from earlier checkpoints during the backward pass.
On the graph, this transformation copies a forward subgraph into the backward phase:
the subgraph rooted at a checkpoint node is duplicated,
and the cross-phase edges from the original subgraph's intermediate nodes are redirected
to the corresponding nodes in the duplicated subgraph.
This eliminates cross-phase edges for the intermediate nodes,
reducing saved activation memory to only the checkpoint tensors.

\noindent\textbf{Quantization.}
Quantization casts a high-precision activation to a lower precision for storage
and casts it back before the backward computation.
On the graph, this transformation is structurally analogous to offloading:
a cross-phase edge $v \to \nabla\!v$ is split into
$v \xrightarrow{\texttt{cast}} v_\text{q} \xrightarrow{\texttt{cast\_back}} v' \to \nabla\!v$,
where $v_\text{q}$ is a new node with reduced precision (e.g., FP8 instead of BF16).
Unlike offloading, quantization does not change the device placement but reduces the per-element memory footprint.
We note that activation quantization is not mathematically equivalent to full-precision training,
but has been empirically validated at scale in production systems
such as DeepSeek-V3~\cite{TODO} and Kimi-K2~\cite{TODO}
with negligible impact on model quality.

All three transformations operate locally on individual nodes or small subgraphs,
and their effects compose naturally:
multiple transformations can be applied to different nodes of the same graph
without global restructuring.
This composability is the foundation for the holistic search
in \S\ref{subsec:graph-holistic}.
And for example, Figure~\ref{fig:case-study} shows the transformed graph for GLM in the actual training.
% We next ground this framework in concrete MoE architectures
% to quantify the activation memory at stake.



==> src/graph-05-graph-runtime.tex <==
% Section 5: Graph Runtime
% 对应 plan/graph_runtime.md + plan/graph_scheduler_dp.md

\section{Graph Runtime}
\label{sec:runtime}

\S\ref{sec:graph} defines the activation-centric compute graph
and formulates activation reduction as composable graph transformations.
This section builds on that abstraction to address three runtime questions:
(1) how much activation memory can each micro batch afford,
(2) which transformations to apply given that budget, and
(3) in what order should the resulting operations execute to minimize latency.
Before each micro batch's forward step, the \sysname{} runtime performs three steps:

\noindent\textbf{Budget calculation} (\S\ref{subsec:budget}):
        determine the per-micro-batch activation memory budget
        based on pipeline phase and current memory usage.
        
\noindent\textbf{Holistic graph transformation} (\S\ref{subsec:graph-holistic}):
        greedily apply graph transformations from \S\ref{subsec:graph-transform}
        until the activation footprint meets the budget,
        with conflict checking to ensure correctness when composing
        heterogeneous strategies.

\noindent\textbf{Overlap scheduling} (\S\ref{subsec:dp}):
        determine the optimal execution order of all operations ---
        including the newly introduced recompute, offload, and cast operators ---
        to maximize compute--communication overlap.

\subsection{Pipeline-Aware Dynamic Memory Budget}
\label{subsec:budget}


\begin{algorithm}[b]
\caption{Pipeline-Aware Memory Budget Allocation}
\label{alg:budget}
\begin{algorithmic}[1]
\Require Total micro batches $B$, warmup count $B_w$,
         GPU capacity $M_{\max}$, min budget $M_0$

\State $\textit{budget}[0 \ldots B{-}1] \gets 0 $
\State $M_{\text{used}} \gets$ non-activation memory usage
\For{$i = 0$ \textbf{to} $B_w - 1$} \Comment{Warmup}
  \State $r \gets B_w - i$
  \State $\textit{budget}[i] \gets (M_{\max} - M_{\text{used}} - r \cdot M_0) / r + M_0$
  \State $\textit{actual} \gets \Call{RunForward}{i, \textit{budget}[i]}$
  \State $\textit{budget}[i] \gets \textit{actual}$
  \State $M_{\text{used}} \mathrel{+}= \textit{actual}$
\EndFor
\For{$i = B_w$ \textbf{to} $B - 1$} \Comment{Steady}
  \State $M_{\text{used}} \mathrel{-}= \textit{budget}[i - B_w]$
  \State $\textit{budget}[i] \gets M_{\max} - M_{\text{used}}$
  \State $\textit{actual} \gets \Call{RunForward}{i, \textit{budget}[i]}$
  \State $\textit{budget}[i] \gets \textit{actual}$
  \State $M_{\text{used}} \mathrel{+}= \textit{actual}$
\EndFor
\end{algorithmic}
\end{algorithm}

The activation memory budget depends on both the pipeline schedule phase
and the actual memory pressure at runtime.
We dynamically compute a per-micro-batch budget that guarantees
all concurrent micro batches fit within GPU memory.

Algorithm~\ref{alg:budget} describes the budget allocation procedure.
Let $B$ denote the total number of micro batches,
$B_w$ the number of warmup batches,
$M_{\max}$ the GPU memory capacity,
and $M_0$ the minimum per-batch activation memory
(achieved under full recomputation, retaining only the block input tensor of size $bsh$).

% \paragraph{Pipeline phases.}
Under pipeline parallelism, the number of in-flight micro batches
(those whose activations reside on GPU) varies over time.
In warmup phase, only forward passes execute;
the number of in-flight batches grows to its maximum $B_{w}$,
and no backward pass releases memory.
In steady phase, forward and backward passes alternate;
the in-flight count stays at $B_{w}$,
but each backward pass frees one batch's activations
before the next forward begins.
During warmup (lines 3-9), no backward pass releases memory,
so the budget for each new micro batch is computed by
evenly distributing the remaining capacity among all yet-to-be-launched batches,
while reserving $M_0$ for each to guarantee feasibility.
During the steady phase (lines 10--16), each forward is preceded by a backward
that frees the activations of an earlier micro batch (line 11),
and the freed memory is fully allocated to the incoming batch (line 12).
In both phases, the budget is updated to the actual memory consumed (lines 7, 14),
so that over-estimation in one batch does not cascade into under-allocation for subsequent batches.


\subsection{Holistic Graph Transformation}
\label{subsec:graph-holistic}

% \paragraph{Problem formulation.}
The \textsc{RunForward} call in Algorithm~\ref{alg:budget}
invokes the graph transformation before executing the forward pass.
Its input is the activation-centric graph $G$ of a transformer block
and the memory budget $\textit{budget}[i]$ computed for micro batch $i$.
The goal is to find a set of graph transformations that reduces
the total saved activation memory below $\textit{budget}[i]$
while minimizing the additional computational and communication overhead.

We solve this problem with a greedy iterative algorithm (Algorithm~\ref{alg:transform}).
At each iteration, we evaluate the memory reduction of every candidate single-node transformation
on the current graph, select the one with the largest reduction,
verify that it does not conflict (detailed below) with previously applied transformations,
and apply it if valid.
The algorithm terminates when the memory budget is satisfied.
The potential memory reduction is re-evaluated at each iteration,
since applying one transformation may change the benefit of subsequent ones
(e.g., recomputing a subgraph makes offloading its intermediate nodes unnecessary).

\begin{algorithm}[t]
\caption{Holistic Graph Transformation}
\label{alg:transform}
\begin{algorithmic}[1]
\Require Activation graph $G$, memory budget $M$
\Ensure Transformed graph $G'$ with activation memory $\leq M$
\State $\textit{mem} \gets \Call{ActivationMemory}{G}$
\If{$\textit{mem} \leq M$}
  \State \Return $G$ \Comment{No transformation needed}
\EndIf
\While{$\textit{mem} > M$}
  \State $t^* \gets$ available transform primitive on $G$ with largest memory reduction 
  % \State Evaluate memory delta for each candidate transform on $G$
  % \State Select candidate $t^*$ with largest memory reduction
  \If{\Call{Conflict}{$G$, $t^*$}}
    \State Mark $t^*$ as unavailable; \textbf{continue}
  \EndIf
  \State $G \gets \Call{Apply}{G, t^*}$
  \State $\textit{mem} \gets \Call{ActivationMemory}{G}$
\EndWhile
\State \Return $G$
\end{algorithmic}
\end{algorithm}

% \paragraph{Conflicting transformations.}
We now explain why conflict checking is necessary.
Existing activation reduction systems typically employ only one or two strategies in isolation
and do not encounter conflicts between them.
When composing all three strategies holistically, however,
we find that independently valid transformations can interact to produce redundant storage,
a phenomenon we term \textbf{conflicting transformations}.

The root cause is that a single logical tensor may have multiple references in the graph
(i.e., it serves as input to multiple operators).
When different transformations are applied to different references of the same tensor,
inconsistencies arise.
We identify two common patterns: \textcolor{red}{TODO: add figure}

\noindent\textit{Case 1: Multi-precision conflict.}
The same logical tensor is transformed into different precisions at different references,
causing multiple copies to coexist.
For example, the MoE layer input $m_0$ serves as input to both the router
(which requires FP32 for numerical stability)
and the shared expert (which uses BF16 or FP8).
If quantization is applied independently to each reference,
both an FP32 and an FP8 copy are stored, increasing rather than reducing total memory.

\noindent\textit{Case 2: Multi-device conflict.}
The same logical tensor is offloaded at one reference but remains on GPU at another,
so the GPU copy cannot be freed.
For example, the core attention output $a_7$ is consumed by \texttt{attn\_out\_proj};
if offloading is applied to the attention output but the projection input
(logically the same tensor) is not offloaded,
the GPU tensor persists and the offload yields no GPU memory savings.

% \paragraph{Conflict detection.}
To detect these conflicts, we perform a lifetime analysis pass
after each candidate transformation.
The analysis traces each newly created node back to its original node in the untransformed graph
and checks whether multiple transformed copies of the same logical tensor coexist
with inconsistent precision or device placement.
If a conflict is detected, the candidate transformation is rejected.
Since the greedy algorithm selects transformations in decreasing order of memory benefit,
a conflicting candidate always conflicts with a previously applied transformation
that yields a larger reduction;
skipping the current candidate is therefore always preferable to reverting the earlier, more beneficial one.

% \paragraph{Transition to runtime scheduling.}
The output of Algorithm~\ref{alg:transform} is a transformed graph $G'$
that satisfies the memory budget while incorporating recomputation, offloading, and quantization operations.
This graph is then passed to the runtime scheduler (\S\ref{subsec:dp}),
which determines the optimal execution order of all operations ---
including the newly introduced reload, recompute, and cast operators ---
to minimize end-to-end latency.

\subsection{Dual-Batch Overlap Scheduling}
\label{subsec:dp}

During the steady phase of pipeline parallelism,
each GPU simultaneously executes the forward pass of one micro batch
and the backward pass of another.
These two micro batches are data-independent,
creating an opportunity to interleave their operations
across the GPU's computation and communication streams
to hide the latency introduced by activation reduction.
We formulate this as a makespan-minimization problem
and solve it with a lightweight dynamic programming algorithm.

\noindent\textbf{Problem formulation.}
We model the GPU as two parallel streams:
a \textit{computation} stream (GEMM, core attention, etc.)
and a \textit{communication} stream (alltoall, offload/reload, etc.).
The input consists of the transformed graphs
for two concurrent micro batches:
$G_f$ (forward) and $G_b$ (backward).
The goal is to assign all operations from both graphs to the two streams
so as to minimize the makespan $T^* = \max(t_c^{\text{end}}, t_m^{\text{end}})$,
where $t_c^{\text{end}}$ and $t_m^{\text{end}}$ are the completion times
of the computation and communication streams, respectively.

\noindent\textbf{Stage decomposition.}
To keep the DP state space compact,
we partition each graph into \textit{stages} at alltoall boundaries.
Each stage is a contiguous group of operators on the same stream,
with cost equal to the sum of its constituent operator costs.
Within each phase, stages execute in a fixed order:
$F_0 \!\to\! F_1 \!\to\! F_2 \!\to\! F_3$
and
$B_0 \!\to\! B_1 \!\to\! B_2 \!\to\! B_3$,
where computation and communication stages alternate,
creating natural overlap opportunities.

\noindent\textbf{Flexible operations.}
Beyond the fixed stage chains,
two classes of operations have relaxed scheduling constraints:

\noindent\textit{Weight-gradient operations:} $W_0, W_1, \ldots, W_{N_w - 1}$
compute gradients with respect to trainable weights.
They execute on the computation stream
and have no downstream consumers in the backward pass
(their outputs feed the optimizer).
$W_k$ is schedulable once backward stage $\mathit{dep}_w(k)$ has completed,
providing the required input gradient.
Weight-gradient operations can therefore be \textit{arbitrarily delayed}
and inserted into any computation gap after their dependency is met.

\noindent\textit{Restore operations:} $R_0, R_1, \ldots, R_{N_r - 1}$
encompass recomputation (comp stream), reload from CPU (comm stream),
and precision cast-back (comp stream).
Their inputs are already available from the forward pass or CPU memory,
so they have no backward-phase predecessors
and can be \textit{arbitrarily advanced}.
However, $R_l$ must complete before backward stage $\mathit{dep}_r(l)$ begins,
since that stage consumes $R_l$'s output.

The large number of flexible operations could make the search space intractable.
However, by an exchange argument, ordering weight-gradient ops
by $\mathit{dep}_w(k)$ ascending (earliest-satisfiable first)
and restore ops by $\mathit{dep}_r(l)$ ascending (earliest-deadline first)
is optimal within each class.
Fixing these canonical orderings reduces the problem
to deciding \textit{when} to insert each operation,
not \textit{in what order}.

\noindent\textbf{Dynamic programming formulation.}
With the relative order of flexible operations fixed,
the scheduling state is fully described by how many operations of each type
have been completed.

\begin{table*}[t]
\centering
\small
\caption{MoE model configurations.}
\label{tab:models}
\begin{tabular}{ccccccccccccc}
\toprule
\textbf{Model} & \textbf{Hidden} & \textbf{MoE Hidden} & \textbf{\#E} & \textbf{Top-$K$} & \textbf{\#Heads} & \textbf{Head Dim} & \textbf{\#GPUs} & \textbf{DP} & \textbf{TP} & \textbf{EP} & \textbf{PP} \\
\midrule
GLM-188B-A20B & 7168 & 4096 & 64 & 4 & 64 & 112 & 128 & 16 & 2 & 32 & 4(vp2) \\
GLM-319B-A30B & 8192 & 4096 & 96 & 6 & 64 & 128 & 256 & 16 & 2 & 32 & 8(vp1) \\
GLM-423B-A30B  & 8192 & 4096 & 128 & 6 & 64 & 128 & 512 & 32 & 2 & 64 & 8(vp2) \\
GLM-629B-A30B  & 8192 & 4096 & 192 & 6 & 64 & 128 & 1024 & 64 & 2 & 64 & 8(vp2) \\
GLM-783B-A35B  & 8192 & 5120 & 192 & 6 & 64 & 128 & 2048 & 128 & 2 & 64 & 8(vp1) \\
GLM-835B-A30B  & 8192 & 4096 & 256 & 6 & 64 & 128 & 4096 & 256 & 2 & 128 & 8(vp2) \\
GLM-1041B-A35B  & 8192 & 5120 & 256 & 6 & 64 & 128 & 8192 & 512 & 2 & 128 & 8(vp2) \\
GLM-1041B-A35B  & 8192 & 5120 & 256 & 6 & 64 & 128 & 12288 & 768 & 2 & 128 & 8(vp2) \\
% TODO: fill in model configs
\bottomrule
\end{tabular}
\end{table*}

\noindent\textit{DP State.}
A state is a 4-tuple $(i, j, k, l)$ where
$i \in \{0, \ldots, N_f\}$ forward stages,
$j \in \{0, \ldots, N_b\}$ backward stages,
$k \in \{0, \ldots, N_w\}$ weight-gradient ops,
and $l \in \{0, \ldots, N_r\}$ restore ops have been completed.

\noindent\textit{DP Value.}
Each state stores a Pareto-optimal set of 4-tuples:
\[
  P(i,j,k,l) = \text{Pareto set of } (t_c,\; t_m,\; t_{fr},\; t_{br}),
\]
where $t_c$ and $t_m$ are the earliest free times of the computation
and communication streams,
and $t_{fr}$ and $t_{br}$ are the data-ready times
for the next forward and backward stages, respectively.
A point $p$ dominates $q$ (written $p \preceq q$) iff
$p.t_c \le q.t_c \,\land\, p.t_m \le q.t_m
\,\land\, p.t_{fr} \le q.t_{fr} \,\land\, p.t_{br} \le q.t_{br}$.

% \paragraph{Boundary conditions.}
The initial state is $P(0,0,0,0) = \{(0,0,0,0)\}$.
At the terminal state $(N_f, N_b, N_w, N_r)$,
the optimal makespan is
\[
  T^* = \min_{(t_c, t_m, \cdot\,, \cdot) \,\in\, P} \max(t_c, t_m).
\]

% \paragraph{Why 4D?}
% A na\"ive 2D formulation using only $(t_c, t_m)$ conflates stream occupancy
% with data readiness.
% When a flexible operation (e.g., $W_k$) is inserted
% between two consecutive stages on the same stream,
% the 2D formulation incorrectly delays the next stage
% by the flexible operation's cost,
% missing the opportunity to overlap it on the other stream.
% The additional dimensions $t_{fr}$ and $t_{br}$
% record when the last forward and backward stages actually completed,
% independent of subsequent flexible operations on the same stream.
% Table~\ref{tab:2d-vs-4d} illustrates this with a concrete example.

% \begin{table}[t]
% \centering
% \small
% \caption{2D vs.\ 4D state after scheduling $F_0$ (comp, cost\,=\,10),
% then $W_0$ (comp, cost\,=\,3), before $F_1$ (comm, cost\,=\,5).
% The 2D approach over-estimates $F_1$'s start by the cost of $W_0$,
% missing the parallel execution of $W_0$ (comp) and $F_1$ (comm).}
% \label{tab:2d-vs-4d}
% \begin{tabular}{lcc}
% \toprule
% & \textbf{2D} $(t_c, t_m)$ & \textbf{4D} $(t_c, t_m, t_{fr}, t_{br})$ \\
% \midrule
% After $F_0$  & $(10, 0)$    & $(10,\; 0,\; 10,\; 0)$ \\
% After $W_0$  & $(13, 0)$    & $(13,\; 0,\; \mathbf{10},\; 0)$ \\
% $F_1$ starts & $\max(0, 13) = 13$ & $\max(0, \mathbf{10}) = 10$ \\
% $F_1$ ends   & $18$ & $15$ \\
% \bottomrule
% \end{tabular}
% \end{table}

\noindent\textit{Transitions.}
From each state $(i,j,k,l)$ and Pareto point $(t_c, t_m, t_{fr}, t_{br})$,
four transitions are possible.
Let $\sigma(X) \in \{\text{comp}, \text{comm}\}$ denote the stream type
and $c(X)$ the cost of stage or operation $X$.
We write $t_\sigma$ for $t_c$ if $\sigma = \text{comp}$
and $t_m$ if $\sigma = \text{comm}$.

\smallskip\noindent\textit{T1. Schedule forward stage $F_i$}
$\to (i\!+\!1, j, k, l)$.
\quad Pre: $i < N_f$.
\[
  \mathit{exit} = \max(t_\sigma,\, t_{fr}) + c(F_i).
\]
Update $t_\sigma \gets \mathit{exit}$ and $t_{fr} \gets \mathit{exit}$.

\smallskip\noindent\textit{T2. Schedule backward stage $B_j$}
$\to (i, j\!+\!1, k, l)$.
\quad Pre: $j < N_b$ and $l \ge \mathit{req}_r(j)$.
\[
  \mathit{exit} = \max(t_\sigma,\, t_{br}) + c(B_j).
\]
Update $t_\sigma \gets \mathit{exit}$ and $t_{br} \gets \mathit{exit}$.
Here $\mathit{req}_r(j) = |\{l' : \mathit{dep}_r(l') \le j\}|$
ensures all restore ops needed by $B_j$ are complete.

\smallskip\noindent\textit{T3. Schedule weight-gradient $W_k$}
$\to (i, j, k\!+\!1, l)$.
\quad Pre: $k < N_w$ and $j \ge \mathit{dep}_w(k)$.
\[
  \mathit{exit} = t_c + c(W_k).
\]
Update $t_c \gets \mathit{exit}$; $t_{fr}$ and $t_{br}$ unchanged.

\smallskip\noindent\textit{T4. Schedule restore operation $R_l$}
$\to (i, j, k, l\!+\!1)$.
\quad Pre: $l < N_r$.
\[
  \mathit{exit} = t_\sigma + c(R_l).
\]
Update $t_\sigma \gets \mathit{exit}$; $t_{fr}$ and $t_{br}$ unchanged.

% \paragraph{Shared expert parallelism.}
% The shared expert path branches from the same input as the MoE gate
% and merges at the final residual addition (\texttt{res\_ffn}).
% Its operators are data-independent of the alltoall dispatch/combine path
% and can overlap with communication stages.
% We model shared expert operations as a forward flexible group ---
% analogous to weight-gradient operations but in the forward phase ---
% adding a fifth state dimension $m \in \{0, \ldots, N_{\mathit{se}}\}$
% (number of shared expert ops completed).
% The constraint is that all shared expert ops must finish
% before the final forward residual stage.
% With $N_{\mathit{se}} \le 4$ in practice,
% the state space grows by a factor of at most 5,
% and total work remains under 10\,ms.

\noindent\textbf{Complexity and memoization.}
The number of DP states is
$(N_f\!+\!1)(N_b\!+\!1)(N_w\!+\!1)(N_r\!+\!1)$.
For a typical MoE Transformer with
$N_f = N_b = 4$, $N_w = 10$, $N_r = 10$:
\[
  |\text{States}| = 5 \times 5 \times 11 \times 11 = 3{,}025.
\]
Each state processes its Pareto set ($|P| < 100$ empirically)
with 4 transitions, giving approximately $1.2$M operations in total.
The algorithm executes in under 1\,ms on a single CPU core ---
negligible compared to the tens of milliseconds of GPU computation it schedules.

Moreover, neither graph transformation nor DP scheduling
needs to be recomputed from scratch at every iteration.
Both algorithms are fully determined by the memory budget:
graph transformation selects strategies for a given budget,
and the DP schedules the resulting graph.
We therefore memoize results keyed by (discretized) budget value.
In practice, memory budgets exhibit strong temporal locality ---
the pipeline phase repeats every $B$ micro batches,
and MoE imbalance rates are stable for the majority of iterations ---
so most iterations hit the cache and skip both algorithms entirely.
This reduces the amortized overhead to near zero.


==> src/tikz/graph-ops.tex <==
\begin{tikzpicture}[
  nd/.style={draw, rounded corners=1.5pt, minimum height=1.15em,
             inner sep=1.5pt, font=\footnotesize},
  fwd/.style={nd, fill=blue!10},
  bwd/.style={nd, fill=red!10},
  cpunode/.style={nd, fill=green!18},
  lpnode/.style={nd, fill=orange!20},
  renode/.style={nd, fill=blue!10, densely dashed},
  >=stealth,
  arr/.style={->},
  sav/.style={->, densely dashed, thick},
  phl/.style={dotted, gray},
]
% ---- phase labels (top) ----
\node[font=\scriptsize\itshape, gray] at (0.6, 0.65) {fwd};
\node[font=\scriptsize\itshape, gray] at (2.0, 0.65) {bwd};
\node[font=\scriptsize\itshape, gray] at (4.7, 0.65) {fwd};
\node[font=\scriptsize\itshape, gray] at (6.7, 0.65) {bwd};

% ===== (a) Offload =====
\node[font=\footnotesize\bfseries, anchor=east] at (-0.3, 0) {(a)};
% before
\node[fwd]  (a1v) at (0.6, 0) {$v$};
\node[bwd]  (a1g) at (2.0, 0) {$\nabla\!v$};
\draw[sav] (a1v) -- (a1g);
\draw[phl] (1.3, 0.5) -- (1.3, -0.45);
% arrow
\node at (3.0, 0) {$\Rightarrow$};
% after
\node[fwd]     (a2v) at (3.9, 0) {$v$};
\node[cpunode]  (a2c) at (5.3, 0) {$v_{\!c}$};
\node[bwd]     (a2g) at (6.9, 0) {$\nabla\!v$};
\draw[arr] (a2v) -- node[above, font=\scriptsize] {offload} (a2c);
\draw[arr] (a2c) -- node[above, font=\scriptsize] {reload} (a2g);
\draw[phl] (4.6, 0.5) -- (4.6, -0.45);
\node[font=\tiny, gray, below=0.05em] at (a2c.south) {CPU};

% ===== (b) Recompute =====
\node[font=\footnotesize\bfseries, anchor=east] at (-0.3, -1.35) {(b)};
% before
\node[fwd]  (b1x) at (0.15, -1.35) {$x$};
\node[fwd]  (b1v) at (1.15, -1.35) {$v$};
\node[bwd]  (b1g) at (2.15, -1.35) {$\nabla\!v$};
\draw[arr] (b1x) -- node[above, font=\scriptsize] {\textit{op}} (b1v);
\draw[sav] (b1v) -- (b1g);
\draw[phl] (1.65, -0.85) -- (1.65, -1.85);
% arrow
\node at (3.0, -1.35) {$\Rightarrow$};
% after
\node[fwd]    (b2x) at (3.9, -1.35) {$x$};
\node[renode] (b2v) at (5.8, -1.35) {$v'$};
\node[bwd]    (b2g) at (6.9, -1.35) {$\nabla\!v$};
\draw[sav] (b2x) -- node[above, font=\scriptsize] {\textit{op}} (b2v);
\draw[arr] (b2v) -- (b2g);
\draw[phl] (4.6, -0.85) -- (4.6, -1.85);
\node[font=\tiny, gray, below=0.05em] at (b2v.south) {recomp};

% ===== (c) Quantization =====
\node[font=\footnotesize\bfseries, anchor=east] at (-0.3, -2.7) {(c)};
% before
\node[fwd]  (c1v) at (0.6, -2.7) {$v$};
\node[bwd]  (c1g) at (2.0, -2.7) {$\nabla\!v$};
\draw[sav] (c1v) -- (c1g);
\draw[phl] (1.3, -2.2) -- (1.3, -3.15);
% arrow
\node at (3.0, -2.7) {$\Rightarrow$};
% after
\node[fwd]    (c2v) at (3.9, -2.7) {$v$};
\node[lpnode] (c2q) at (5.3, -2.7) {$v_{\!q}$};
\node[bwd]    (c2g) at (6.9, -2.7) {$\nabla\!v$};
\draw[arr] (c2v) -- node[above, font=\scriptsize] {cast} (c2q);
\draw[arr] (c2q) -- node[above, font=\scriptsize] {decast} (c2g);
\draw[phl] (4.6, -2.2) -- (4.6, -3.15);
\node[font=\tiny, gray, below=0.05em] at (c2q.south) {FP8};

% ---- legend ----
\node[fwd, font=\tiny] at (1.0, -3.7) {GPU};
\node[font=\tiny, anchor=west] at (1.4, -3.7) {fwd tensor};
\node[bwd, font=\tiny] at (3.0, -3.7) {GPU};
\node[font=\tiny, anchor=west] at (3.4, -3.7) {bwd tensor};
\node[font=\tiny, anchor=west] at (5.0, -3.7) {\tikz\draw[densely dashed, thick, ->] (0,0) -- (0.6,0);};
\node[font=\tiny, anchor=west] at (5.7, -3.7) {saved};
\end{tikzpicture}

==> src/tikz/system-overview.tex <==
% System Overview Figure (standalone, A4 single-column, footnotesize)
% 对应 plan/system_overview_figure.md

% ── colour palette ──
\definecolor{inputfill}{RGB}{255,243,224}    % warm orange tint for inputs
\definecolor{offlinefill}{RGB}{240,240,240}  % light grey for offline zone
\definecolor{onlinefill}{RGB}{228,240,255}   % light blue for online zone
\definecolor{stepfill}{RGB}{255,255,255}     % white for step boxes
\definecolor{loopfill}{RGB}{245,245,255}     % faint violet for loop box
\definecolor{fwdcolor}{RGB}{66,133,244}      % blue for fwd stages
\definecolor{bwdcolor}{RGB}{219,68,55}       % red  for bwd stages
\definecolor{arrowgray}{RGB}{80,80,80}

\begin{tikzpicture}[
    >=Stealth,
    every node/.style={font=\footnotesize},
    box/.style={
      draw, rounded corners=3pt, minimum height=0.8cm,
      align=center, inner sep=6pt
    },
    inputbox/.style={box, fill=inputfill, minimum width=3.2cm, text width=2.8cm},
    stepbox/.style={
      draw, rounded corners=4pt, fill=stepfill,
      inner sep=8pt, text width=4.2cm, align=center
    },
    zonelabel/.style={
      font=\footnotesize\bfseries, anchor=north west, text=black!70
    },
    arrstyle/.style={->, thick, color=arrowgray},
    dasharr/.style={->, thick, dashed, color=arrowgray},
  ]
\footnotesize

  % ====================================================================
  %  INPUT BOXES  (top)
  % ====================================================================
  \node[inputbox] (hw)  {Cluster Hardware\\Info};
  \node[inputbox, right=1.8cm of hw] (model) {MoE Model\\Architecture};

  % ====================================================================
  %  OFFLINE ZONE
  % ====================================================================
  % -- inner content first --
  \node[box, below=1.2cm of $(hw.south)!0.5!(model.south)$,
        minimum width=8.6cm, minimum height=1.6cm,
        fill=white, align=center]
    (graphbox) {};

  % fwd / bwd sub-boxes inside graphbox
  \node[box, fill=fwdcolor!12, minimum width=2.8cm, minimum height=0.9cm, text width=2.4cm]
    at ($(graphbox.center)+(-1.8,0)$) (fwd) {Fwd Graph\\[-1pt]{\scriptsize (tensor nodes, op edges)}};
  \node[box, fill=bwdcolor!12, minimum width=2.8cm, minimum height=0.9cm, text width=2.4cm]
    at ($(graphbox.center)+(1.8,0)$) (bwd) {Bwd Graph\\[-1pt]{\scriptsize (auto-derived)}};
  \draw[arrstyle] (fwd) -- node[above, font=\scriptsize]{auto derive} (bwd);

  % graphbox title
  \node[anchor=south, font=\footnotesize\itshape, yshift=1pt]
    at (graphbox.north) {Activation-Centric Compute Graph};

  % -- offline zone background --
  \begin{scope}[on background layer]
    \node[fit=(graphbox), inner sep=14pt, rounded corners=6pt,
          draw=black!30, dashed, fill=offlinefill] (offline) {};
  \end{scope}
  \node[zonelabel] at (offline.north west) {\quad Offline, one-time \;\;(\S4.0--4.1)};

  % -- arrows from inputs --
  \coordinate (midtop) at ($(hw.south)!0.5!(model.south)$);
  \draw[arrstyle] (hw.south)    |- ++(0,-0.35) -| ($(midtop)$)
        -- (graphbox.north -| midtop)
        node[midway, right, font=\scriptsize]{};
  \draw[arrstyle] (model.south) |- ++(0,-0.35) -| ($(midtop)$);

  % ====================================================================
  %  ONLINE ZONE
  % ====================================================================

  % --- Step 1 -----------------------------------------------------------
  \node[stepbox, below=2.8cm of offline.south, xshift=-5.2cm,
        text width=3.6cm, minimum height=3.8cm] (step1) {};

  \node[anchor=north, font=\footnotesize\bfseries] at (step1.north)
    {Step 1 (\S5.1)};
  \node[anchor=north, yshift=-3mm, font=\footnotesize, text width=3.4cm, align=center]
    at ($(step1.north)+(0,-0.35)$) {Memory Budget\\Calculation};
  \node[anchor=south, yshift=4mm, font=\scriptsize, text width=3.4cm, align=center,
        text=black!60]
    at (step1.south)
    {$\mathit{budget} = f(\text{on-fly batches},$\\
     $\text{memory},\; \text{imbalance})$};

  % input / output labels for step 1
  \node[anchor=south west, font=\sffamily\tiny, text=black!50]
    at ($(step1.north west)+(0.1, 0.15)$) {%
      \begin{tabular}{@{}l@{}}
        \textbf{in:} mb\_id, pp stage,\\
        \quad GPU mem, imbalance
      \end{tabular}};
  \node[anchor=north west, font=\sffamily\tiny, text=black!50]
    at ($(step1.south west)+(0.1, -0.1)$) {\textbf{out:} memory budget};

  % --- Step 2 -----------------------------------------------------------
  \node[stepbox, right=0.7cm of step1,
        text width=4.6cm, minimum height=3.8cm] (step2) {};

  \node[anchor=north, font=\footnotesize\bfseries] at (step2.north)
    {Step 2 (\S4.2--4.3)};
  \node[anchor=north, yshift=-3mm, font=\footnotesize, text width=4.4cm, align=center]
    at ($(step2.north)+(0,-0.35)$) {Graph Transformation};

  % greedy loop sub-box
  \node[draw, rounded corners=2pt, fill=loopfill,
        inner sep=4pt, font=\scriptsize, text width=3.8cm, align=left,
        below=0.95cm of step2.north] (loop)
    {Greedy loop:\\
     evaluate $\to$ select best\\
     transform $\to$ conflict check\\
     $\circlearrowleft$ until budget met};

  % strategy tags
  \node[draw, rounded corners=2pt, fill=fwdcolor!10,
        font=\sffamily\tiny, inner sep=2pt,
        below=2pt of loop.south west, anchor=north west] (tag1) {offload};
  \node[draw, rounded corners=2pt, fill=fwdcolor!10,
        font=\sffamily\tiny, inner sep=2pt,
        right=2pt of tag1] (tag2) {recompute};
  \node[draw, rounded corners=2pt, fill=fwdcolor!10,
        font=\sffamily\tiny, inner sep=2pt,
        right=2pt of tag2] (tag3) {quant};

  % input / output labels for step 2
  \node[anchor=south west, font=\sffamily\tiny, text=black!50]
    at ($(step2.north west)+(0.1, 0.15)$)
    {\textbf{in:} base graph + budget};
  \node[anchor=north west, font=\sffamily\tiny, text=black!50]
    at ($(step2.south west)+(0.1, -0.1)$)
    {\textbf{out:} transformed graph};

  % --- Step 3 -----------------------------------------------------------
  \node[stepbox, right=0.7cm of step2,
        text width=4.6cm, minimum height=3.8cm] (step3) {};

  \node[anchor=north, font=\footnotesize\bfseries] at (step3.north)
    {Step 3 (\S5.2)};
  \node[anchor=north, yshift=-3mm, font=\footnotesize, text width=4.4cm, align=center]
    at ($(step3.north)+(0,-0.35)$) {Dual-Batch Overlap\\DP Scheduling};

  % stream timeline inside step 3
  \coordinate (tl) at ($(step3.center)+(0, -0.15)$);

  % comp stream
  \node[anchor=east, font=\sffamily\tiny] at ($(tl)+(-1.9, 0.35)$) {comp};
  \fill[fwdcolor!60] ($(tl)+(-1.7, 0.2)$)  rectangle +(0.7, 0.3);
  \node[font=\sffamily\tiny, white] at ($(tl)+(-1.35, 0.35)$) {$F_0$};
  \fill[fwdcolor!60] ($(tl)+(-0.5, 0.2)$)  rectangle +(0.7, 0.3);
  \node[font=\sffamily\tiny, white] at ($(tl)+(-0.15, 0.35)$) {$F_2$};
  \fill[bwdcolor!60] ($(tl)+(0.6, 0.2)$)   rectangle +(0.7, 0.3);
  \node[font=\sffamily\tiny, white] at ($(tl)+(0.95, 0.35)$) {$B_1$};
  \fill[bwdcolor!60] ($(tl)+(1.5, 0.2)$)   rectangle +(0.5, 0.3);
  \node[font=\sffamily\tiny, white] at ($(tl)+(1.75, 0.35)$) {$B_3$};

  % comm stream
  \node[anchor=east, font=\sffamily\tiny] at ($(tl)+(-1.9, -0.2)$) {comm};
  \fill[fwdcolor!35] ($(tl)+(-1.0, -0.35)$) rectangle +(0.5, 0.3);
  \node[font=\sffamily\tiny]               at ($(tl)+(-0.75,-0.2)$) {$F_1$};
  \fill[fwdcolor!35] ($(tl)+(0.2, -0.35)$)  rectangle +(0.4, 0.3);
  \node[font=\sffamily\tiny]               at ($(tl)+(0.4, -0.2)$) {$F_3$};
  \fill[bwdcolor!35] ($(tl)+(0.6, -0.35)$)  rectangle +(0.5, 0.3);
  \node[font=\sffamily\tiny]               at ($(tl)+(0.85,-0.2)$) {$B_0$};
  \fill[bwdcolor!35] ($(tl)+(1.3, -0.35)$)  rectangle +(0.5, 0.3);
  \node[font=\sffamily\tiny]               at ($(tl)+(1.55,-0.2)$) {$B_2$};

  % legend below timeline
  \node[font=\sffamily\tiny, fwdcolor, anchor=north west]
    at ($(tl)+(-1.7, -0.55)$) {MB$_f$ (fwd)};
  \node[font=\sffamily\tiny, bwdcolor, anchor=north east]
    at ($(tl)+(2.0, -0.55)$) {MB$_b$ (bwd)};

  % input / output labels for step 3
  \node[anchor=south west, font=\sffamily\tiny, text=black!50]
    at ($(step3.north west)+(0.1, 0.15)$)
    {\textbf{in:} transformed graph};
  \node[anchor=north west, font=\sffamily\tiny, text=black!50]
    at ($(step3.south west)+(0.1, -0.1)$)
    {\textbf{out:} execution schedule};

  % --- Online zone background -------------------------------------------
  \begin{scope}[on background layer]
    \node[fit=(step1)(step2)(step3),
          inner xsep=16pt, inner ysep=22pt,
          rounded corners=6pt, draw=blue!30, dashed, fill=onlinefill]
      (online) {};
  \end{scope}
  \node[zonelabel, text=blue!50!black]
    at (online.north west) {\quad Online, per micro-batch};

  % ====================================================================
  %  OUTPUT BOX
  % ====================================================================
  \node[box, fill=inputfill, minimum width=3.2cm, text width=2.8cm, below=0.9cm of step3.south]
    (output) {Execution\\Schedule};

  % ====================================================================
  %  ARROWS (numbered as in the plan)
  % ====================================================================

  % ① ② inputs -> offline (already drawn above)

  % ③ base graph: offline -> step 2 (long cross-zone arrow, routed on the right)
  \coordinate (route3a) at ($(offline.south -| online.east)+(0.35, 0)$);
  \coordinate (route3b) at ($(step2.north -| online.east)+(0.35, 0.6)$);
  \draw[arrstyle, rounded corners=4pt]
    (graphbox.east) -| (route3a) |- (route3b) -- ($(step2.north)+(0, 0.6)$)
    -- (step2.north)
    node[pos=0.45, right, font=\scriptsize]{base graph};

  % ④ runtime state -> step 1 (dashed, from left)
  \draw[dasharr]
    ($(step1.west)+(-0.8, 0)$) -- (step1.west)
    node[pos=0.0, left, font=\scriptsize, text width=1.6cm, align=right]
      {runtime state\\[-2pt]{\tiny pp stage +}\\[-3pt]{\tiny imbalance rate}};

  % ⑤ step 1 -> step 2
  \draw[arrstyle]
    (step1.east) -- (step2.west)
    node[midway, above, font=\scriptsize]{budget};

  % ⑥ step 2 -> step 3
  \draw[arrstyle]
    (step2.east) -- (step3.west)
    node[midway, above, font=\scriptsize, text width=1.4cm, align=center]
      {transformed\\[-2pt]graph};

  % ⑦ step 3 -> output
  \draw[arrstyle]
    (step3.south) -- (output.north);

\end{tikzpicture}

% \caption{System overview.
% The system takes cluster hardware information and the MoE model architecture as input.
% In the \textbf{offline} stage (\S4), an activation-centric compute graph is constructed
% with forward and auto-derived backward sub-graphs.
% At \textbf{runtime}, for each micro-batch:
% (1)~a memory budget is calculated from pipeline state and MoE imbalance rate (\S5.1);
% (2)~greedy graph transformations (offload, recompute, quantization) are applied
%     subject to conflict checking (\S4.2--4.3);
% (3)~a 4-D Pareto DP scheduler interleaves the forward micro-batch and backward micro-batch
%     on two GPU streams to minimize makespan (\S5.2).}
% \label{fig:system-overview}

